A Large Term Rewrite System Modelling a Pioneering Cryptographic Algorithm

We present a term rewrite system that formally models the Message Authenticator Algorithm (MAA), which was one of the first cryptographic functions for computing a Message Authentication Code and was adopted, between 1987 and 2001, in international standards (ISO 8730 and ISO 8731-2) to ensure the authenticity and integrity of banking transactions. Our term rewrite system is large (13 sorts, 18 constructors, 644 non-constructors, and 684 rewrite rules), confluent, and terminating. Implementations in thirteen different languages have been automatically derived from this model and used to validate 200 official test vectors for the MAA.

==> eptcsdata.tex <==
\providecommand{\firstpage}{129}
\providecommand{\publicationstatus}{H. Hermanns, P. H\"ofner (Eds.): Models for \\
Formal Analysis of Real Systems (MARS 2017)\\
EPTCS 244, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.244.6}{10.4204/EPTCS.244.6}}

